Average distortion embeddings, nonlinear spectral gaps, and a metric John theorem (after Assaf Naor)

We survey various aspects of the theory of nonlinear spectral gaps. In particular, we present a self-contained proof of Naor's average John theorem.

==> README <==
********************************************************************************
* smflatex package version 1.6-20210418
* Copyright (c) Société mathématique de France, 1999-2021
* LaTeX Project Public License (version 1.3c).
********************************************************************************

The Société mathématique de France provides 
a set of classes, packages and bibtex styles
that are used in its publications.
They are based on Ams classes (whose code is sometimes recopied)
and mainly "upward-compatible".

Their main features are
   1. different design, similar to traditional French mathematical journals
   2. new environments for typesetting some informations
in two languages (altabstract, alttitle, altkeywords)
   3. if necessary, use of babel (option french) and desactivation
of some features of french.

The following files are provided in the package (once unpacked)

  smfart.cls
  smfbook.cls	classes for articles and books

  smfenum.sty	package for new alignment style of enumerations
  smfthm.sty	package for simplified definition of theorems

  smfplain.bst
  smfalpha.bst	BibTeX styles 

Are also included:

  smf-edoc.tex	documentation and advices (in english)
  smf-edoc.pdf
  smf-fdoc.tex	documentation et conseils (in french)
  smf-fdoc.pdf

The present distribution is version 1.6-20210418
It consists in minor updates of the 1.5 version and in modifications
of the file names (systematic addition of a smf- prefix) 
in order to be fullfill the requirements of the TeXLive distribution.

The documentation files are slightly outdated.

INSTALLATION : 
  unload these files to $TEXMF/src/latex/smflatex
  compile smflatex.ins 
  move .cls, .sty files to $TEXMF/tex/latex/smflatex
  move .bst files to $TEXMF/bibtex/bst/smflatex
  move .tex and .pdf  files to $TEXMF/doc/latex/smflatex
 
Some additional classes, reserved for internal use of SMF, can be
installed as well,  by manually setting \smftrue in smflatex.ins

This work is subject to the LaTeX Project Public License (version 1.3c).

Maintainer : Antoine Chambert-Loir <antoine.chambert-loir@u-paris.fr>
--
Société mathématique de France
Institut Henri Poincaré
11 rue Pierre et Marie Curie, F-75231 Paris cedex 05
Email : revues@smf.emath.fr
Url : http://smf.emath.fr


